LoVA: Long-form Video-to-Audio Generation

Video-to-audio (V2A) generation is important for video editing and post-processing, enabling the creation of semantics-aligned audio for silent video. However, most existing methods focus on generating short-form audio for short video segment (less than 10 seconds), while giving little attention to the scenario of long-form video inputs. For current UNet-based diffusion V2A models, an inevitable problem when handling long-form audio generation is the inconsistencies within the final concatenated audio. In this paper, we first highlight the importance of long-form V2A problem. Besides, we propose LoVA, a novel model for Long-form Video-to-Audio generation. Based on the Diffusion Transformer (DiT) architecture, LoVA proves to be more effective at generating long-form audio compared to existing autoregressive models and UNet-based diffusion models. Extensive objective and subjective experiments demonstrate that LoVA achieves comparable performance on 10-second V2A benchmark and outperforms all other baselines on a benchmark with long-form video input.

==> asset/intro-chengxin-0912-22_20.tex <==

\section{Introduction}

% Video-to-audio generation, which aims to generate realistic and aligned audio for the input silent video, is an emerging application which can be used for editing video, making sound effects and so on. 
% % Recent years, V2A generation makes great progress along with the improvement of deep generation models. 
% Generally speaking, V2A models can be classified into two groups: The first is autoregressive models like SpecVQGAN \cite{SpecVQGAN_Iashin_2021}, IM2WAV \cite{sheffer2023hear} and FoleyGen \cite{mei2023foleygen}. They take advantage of Transformer to autoregressively generate audio sequence conditioned on video features. Another class is non-autoregressive models, especially diffusion models. For example, DiffFoley \cite{luo2024diff} train a latent diffusion model (LDM) to generate audio spectrum conditioned on CAVP visual features. FoleyCrafter \cite{zhang2024foleycrafter} uses pretrained text-to-audio model and a temporal controller to generate time-aligned audio for video. TiVA \cite{wang2024tiva} leverages the predicted audio layout and semantic latent embeddings as condition to learn a LDM audio generator, which achieves excellent results in both semantic and temporal metrics. 
% % FoleyCrafter utilizes pretained text-to-audio model and train a temporal controller to generate time-aligned audio. Based on commonly used Unet structure as denoiser, these diffusion models demonstrate their strong ability to generate high quality audio in the V2A senario.

Video-to-Audio (V2A) generation, 
aiming to produce synchronized and realistic sound effects for silent videos, 
is widely applied in video editing, sound effect creation and autonomous content enhancement~\cite{ament2014foley}. 
Existing V2A methods have succeeded in generating fixed-length, short audios.
% However, when applied to real-world scenarios, generating audio for long-form videos with variable lengths remains a significant challenge. 
However, generating audio for variable-length, long-form videos in practical applications remains a significant challenge.
These challenges highlight the need for more flexible V2A models that can effectively handle the long-form input videos, as well as a well-established benchmark for long-form V2A generation.



\begin{figure}[htbp]
\centerline{\includegraphics[scale=0.75]{asset/case.pdf}}
\caption{\fontsize{9pt}{11pt} \selectfont Example of the inconsistency phenomenon for current diffusion V2A models when generating long-form (30 seconds) audio. The duration in parentheses denotes each model's generated length per inference. The dotted yellow line denotes the splicing artifacts between adjacent generated sub-audios. }
\label{case}
\end{figure}


Existing V2A models generally fall into two categories: autoregressive models and non-autoregressive models. Autoregressive models, such as SpecVQGAN~\cite{SpecVQGAN_Iashin_2021}, IM2WAV~\cite{sheffer2023hear}, and FoleyGen~\cite{mei2023foleygen}, utilize Transformer-based architectures~\cite{vaswani2017attention} to generate audio sequences with video features as conditions. These models show high quality audio generation performance for short-form fixed-length V2A generation.
However, when being extended to long-form V2A generation, the inference time becomes prohibitively long. 
Most non-autoregressive models are diffusion-based architecture~\cite{ho2020denoising}, like DiffFoley~\cite{luo2024diff}, FoleyCrafter~\cite{zhang2024foleycrafter}, and TiVA~\cite{wang2024tiva}. Taking advantage of sampling strategies, they can efficiently generate high-fidelity short-form audio for input video.  
However, these models mostly untilize UNet~\cite{ronneberger2015u,rombach2022high} as denoiser and are trained on short-form data, thus they may produce suboptimal results when synthesizing long audio sequences~\cite{huang2023make}. This CNN-based architecture generally encounter limitations in long-range relation modeling, due to the intrinsic locality of convolution operations~\cite{chen2021transunet, zhou2021nnformer, hatamizadeh2022unetr}. For audio generation task, UNet structure is not necessary and our experimental results in Section.~\ref{comparison results} also prove the degeneration of UNet when the sequence lengthens. Therefore, due to the limitation of model structure, these models' supported generation length is usually impossible to exceed the length of the training data, or  there will be a obvious deteriorated results.
When handling long-form video input, these models have to divide the video into short clips and generate corresponding audio segments individually. 
As shown in Fig.~\ref{case}, the supported generation length of DiffFoley, TiVA and FoleyCrafter is far less than the required length of video (30 seconds). And their final audios are concatenated by multiple sub-audios from independent denoising process. This method often introduces splicing artifacts and inconsistencies in the final concatenated audio, compromising the coherence compared to the ground truth. In summary, the autoregressive model's slow inference speed and diffusion model's inconsistent generated result restrict existing V2A models to extend to long-form audio generation.
% Besides, prior research \cite{huang2023make} suggests that the UNet backbone trained on fixed-length short audio, may produce suboptimal results when synthesizing long audio sequences.


To address these limitations, we propose LoVA, a video-to-audio generation model designed for long-form video input specifically. To handling long-form videos with variable length, LoVA based on Diffusion Transformer (DiT) structure~\cite{peebles2023scalable} instead of the commonly used UNet-based backbone.
The transformer within DiT, which treats tokens as temporal sequences, aligns well with the temporal nature of audio signals and is capable for capturing long-range dependencies~\cite{huang2018music, dhariwal2020jukebox, borsos2023audiolm}. 
DiT-based models have shown promising performance on generating long-form music and audio given text prompts~\cite{evans2024long,evans2024stable}.
In the long-form V2A tasks, we introduce DiT into LoVA to capture long-form dependencies and maintain coherence over extended periods. 
In addition, to facilitate the development of long-form V2A generation, we build a new benchmark based on UnAV100~\cite{geng2023dense} dataset. Different from commonly used 10-second V2A benchmark VGGSound~\cite{chen2020vggsound}, UnAV100  is composed primarily of untrimmed videos ranging from 10 to 60 seconds in duration. This is the first time that long-form video of variable lengths is introduced into V2A evaluation.

\begin{figure*}[ht]
\centerline{\includegraphics[scale=0.71]{asset/structure3.pdf}}
\caption{ \fontsize{9pt}{11pt} \selectfont Overview of LoVA. In order not to affect the generation quality, UNet diffusion model do the inference by fixed short duration. However, transformer-based DiT block takes sampled noise as temporal sequence, thus can handle arbitrary generated length and do the denoising process integrally.}
\label{fig2}
\end{figure*}

% To build a new benchmark for long-form V2A evaluation, we employ the UnAV100 \cite{geng2023dense} dataset, which is composed primarily of untrimmed videos ranging from 10 to 60 seconds in duration. To adapt 10-second-trained audio classifiers %like VGGish \cite{hershey2017cnn}, PANN \cite{kong2020panns}, and PaSST \cite{koutini2021efficient} Given that the commonly used V2A benchmark, VGGSound \cite{chen2020vggsound}, consists of only 10-second trimmed clips,
% for long-form audio evaluation, we also modify the way of calculating fréchet audio distance~\cite{kilgour2018fr}, inception score, and mean KL divergence. Besides, in long-form V2A generation, it is common for subdivisions of the audio to be generated independently, which can lead to inconsistencies when these segments are combined, as indicated in Fig.~\ref{case}. Additionally, we introduce a new metric called average number of inferences (NumInfer), which can serve as an indicator of potential inconsistencies in generated long-form audios.

LoVA is designed to generate long-form audio clips up to  44.1kHz sampling rate.
Experimental results demonstrate that LoVA performs comparably with existing V2A methods on the 10-second V2A benchmark VGGSound ~\cite{chen2020vggsound}, while significantly outperforming them on the long-form V2A benchmark UnAV100~\cite{geng2023dense} with the fewest number of inferences. 



Overall, our main contributions are as follows:






\begin{itemize}
\item  We raise the issue of long-form V2A generation, point out the gap between existing V2A models and practical applications.
\item We introduce DiT into V2A area and propose a new model, LoVA, which is better suited for generating long-form high-sampling-rate audio than existing methods.
\item Experimental results demonstrate that LoVA achieves comparable performance on the 10-second V2A benchmark and get SOTA results on the long-form benchmark. Demo samples are available at https://ceaglex.github.io/LoVA.github.io/. 
\end{itemize}

% To ensure a fair comparison with other V2A models, we train LoVA on the 10-second dataset. Experimental results demonstrate that LoVA performs comparably on the 10-second benchmark while significantly outperforming other models on the long-form V2A benchmark UnAV100 across all metrics. Our model produces high-quality long-form audio with the fewest inference times and highest sampling rate, underscoring the effectiveness of the DiT structure in long-form V2A generation.
% For a fair comparison, we train our model on 10-second dataset same as other V2A models. Experiment results show that LoVA achieves comparable performance with currents V2A models on 10-second benchmark VGGSound. On long-form V2A benchmark UnAV100, our model can generate long-form audio with the fewest average infer times, the highest sampling rate and the best quality. Comprehensive experiments demonstrate the effectiveness of LoVA and its DiT structure.
